Fighting the COVID-19 Infodemic in Social Media: A Holistic Perspective and a Call to Arms

With the outbreak of the COVID-19 pandemic, people turned to social media to read and to share timely information including statistics, warnings, advice, and inspirational stories. Unfortunately, alongside all this useful information, there was also a new blending of medical and political misinformation and disinformation, which gave rise to the first global infodemic. While fighting this infodemic is typically thought of in terms of factuality, the problem is much broader as malicious content includes not only fake news, rumors, and conspiracy theories, but also promotion of fake cures, panic, racism, xenophobia, and mistrust in the authorities, among others. This is a complex problem that needs a holistic approach combining the perspectives of journalists, fact-checkers, policymakers, government entities, social media platforms, and society as a whole. Taking them into account we define an annotation schema and detailed annotation instructions, which reflect these perspectives. We performed initial annotations using this schema, and our initial experiments demonstrated sizable improvements over the baselines. Now, we issue a call to arms to the research community and beyond to join the fight by supporting our crowdsourcing annotation efforts.

==> sections/annotation_questions_long.tex <==
\subsubsection{\textbf{Question 1:} Does the tweet contain a verifiable factual claim?}

A \emph{verifiable factual claim} is a sentence claiming that something is true, and this can be verified using factual verifiable information such as statistics, specific examples, or personal testimony. 
% Some positive examples (factual claims; this is NOT an exhaustive list): 
Factual claims include the following:\footnote{Inspired by \citep{DBLP:journals/corr/abs-1809-08193}.}
\begin{itemize}
    \itemsep-0.2em 
    \item Stating a definition; 
    \item Mentioning quantity in the present or the past;
    \item Making a verifiable prediction about the future; 
    \item Statistics or specific examples;
    \item Personal experience or statement (e.g., \textit{``I spent much of the last decade working to develop an \#Ebola treatment.''})
    \item Reference to laws, procedures, and rules of operation;
    \item References (e.g., URL) to images or videos (e.g., \textit{``This is a video showing a hospital in Spain.''});
    \item Statements which can be technically classified as questions, but in fact contain a verifiable claim based on the criteria above (e.g., \textit{``Hold on - \#China Communist Party now denying \#CoronavirusOutbreak originated in China? This after Beijing's catastrophic mishandling of the virus has caused a global health crisis?''})
    \item Statements about correlation or causation. Such a correlation or causation needs to be explicit, i.e., sentences like \textit{``This is why the beaches haven't closed in Florida. https://t.co/8x2tcQeg21''} is not a claim because it does not explicitly say why, thus it is not verifiable. 
\end{itemize}
Tweets containing personal opinions and preferences are not factual claims. 
% Some negative examples: personal opinions and preferences. 
Note that if a tweet is composed of multiple sentences or clauses, at least one full sentence or clause needs to be a claim in order for the tweet to contain a factual claim. If a claim exist in a sub-sentence or sub-clause, then the tweet is not considered to have a factual claim. 
For example, \textit{``My new favorite thing is Italian mayors and regional presidents LOSING IT at people violating quarantine''} is not a claim -- it is in fact an opinion. Moreover, if we consider \textit{``Italian mayors and regional presidents LOSING IT at people violating quarantine''} it would be a claim. In addition, when answering this question, annotators should not open the tweet URL. 
%\textcolor{blue}{ND: We need to explain the rational behind not doing this just for Question 1}. 
Since this is a binary decision task, the answer of this question consists of two labels as defined below. 

\noindent\textbf{Labels:}
\begin{itemize}
    \itemsep-0.2em 
    \item \lbl{YES:} if it contains a verifiable factual claim;
    \item \lbl{NO:} if it does not contain a verifiable factual claim;
    \item \lbl{Don't know or can't judge:} the content of the tweet does not have enough information to make a judgment. It is recommended to categorize the tweet using this label when the content of the tweet is not understandable at all. For example, it uses a language (i.e., non-English) or references that it is difficult to understand;
\end{itemize}

\noindent \textbf{Examples:}

\begin{enumerate}
    \item \textit{Please don't take hydroxychloroquine (Plaquenil) plus Azithromycin for \#COVID19 UNLESS your doctor prescribes it. Both drugs affect the QT interval of your heart and can lead to arrhythmias and sudden death, especially if you are taking other meds or have a heart condition.} \\
    \textbf{Label:} \lbl{YES} \\
    \textbf{Explanation:} There is a claim in the text.
    \item \textit{Saw this on Facebook today and it’s a must read for all those idiots clearing the shelves \#coronavirus \#toiletpapercrisis \#auspol} \\
    \textbf{Label:} \lbl{NO} \\
    \textbf{Explanation:} There is no claim in the text.
\end{enumerate}

% \subsection{False Information}

\subsubsection{\textbf{Question 2:} To what extent does the tweet appear to contain false information?} 

The stated claim may contain false information. This question labels the tweets with the categories mentioned below. \textit{False Information} appears on social media platforms, blogs, and news-articles to deliberately misinform or deceive the readers~\citep{kumar2018false}.
% \footnote{https://www.webwise.ie/teachers/what-is-fake-news/} 

\noindent\textbf{Labels:}
The labels for this question are defined with a five point Likert scale~\citep{albaum1997likert}. A higher value means that it is more likely to be false: 

\begin{enumerate}
\itemsep-0.2em 
\item \lbl{NO, definitely contains no false information}
\item \lbl{NO, probably contains no false information}
\item \lbl{not sure}
\item \lbl{YES, probably contains false information}
\item \lbl{YES, definitely contains false information}
\end{enumerate}


To answer this question, it is recommended to open the link of the tweet and to look for additional information for the veracity of the claim identified in question 1. For example, if the tweet contains a link to an article from a reputable information source (e.g., Reuters, Associated Press, France Press, Aljazeera English, BBC), then the answer could be ``\dots~contains no false info''.

\noindent \textbf{Examples:}
\begin{enumerate}
\item \textit{``Dominican Republic found the cure for Covid-19 https://t.co/1CfA162Lq3''}
\\
\textbf{Label:}\enspace\lbl{5.}\,\lbl{YES, definitely contains false information}
\\
\textbf{Explanation:} This is not correct information at the time of this tweet is posted. 

\item \textit{This is Dr. Usama Riaz. He spent past weeks screening and treating patients with Corona Virus in Pakistan. He knew there was no PPE. He persisted anyways. Today he lost his own battle with coronavirus but he gave life and hope to so many more. KNOW HIS NAME \img{figures/emoticon_example.png} https://t.co/flSwhLCPmx}
\\
\textbf{Label:}\enspace\lbl{2.}\,\lbl{NO, probably contains no false info}
\\
\textbf{Explanation:} The content of the tweet states correct information. 


\end{enumerate}

% \subsection{Interest to General Public}
\subsubsection{\textbf{Question 3:} Will the tweet's claim have an effect on or be of interest to the general public?}

Most often people do not make interesting claims, which can be verified by our general knowledge. For example, though \textit{``The sky is blue''} is a claim, it is not interesting to the general public. In general, topics such as healthcare, political news, and current events are of higher interest to the general public. Using the five point Likert scale the labels are defined below.
%%https://papyr.com/hypertextbooks/comp2/factual.htm

\noindent\textbf{Labels:}

\begin{enumerate}
\itemsep-0.2em 
\item \lbl{NO, definitely not of interest}
\item \lbl{NO, probably not of interest}
\item \lbl{not sure}
\item \lbl{YES, probably of interest}
\item \lbl{YES, definitely of interest}
\end{enumerate}

\noindent \textbf{Examples:} 
\begin{enumerate}
    \item \textit{Germany is conducting 160k Covid-19 tests a week. It has a total 35k ventilators, 10k ordered to be made by the govt. It has converted a new 1k bed hospital in Berlin.   It’s death rate is tiny bcos it’s mass testing allows quarantine and bcos it has fewer non reported cases.} \\
    \textbf{Label:}\enspace\lbl{4.}\,\lbl{YES: probably of interest} \\
    \textbf{Explanation:} This information is relevant and of high interest for the general population as it reports how a country deals with COVID-19.
    
    % \item \textit{I feel like a broken record but I’ll say it again...surgical masks WILL NOT prevent you from getting \#COVID19 but they can keep you from spreading germs if you have a cough. \#tweetiatrician \#CoronaOutbreak \#pediatiktok} %[https://twitter.com/NicoleB_MD/status/1235198085367844869]
    % \\
    % \textbf{Label:}\enspace\lbl{5.}\,\lbl{YES, definitely of interest}
    
    \item \textit{Fake news peddler Dhruv Rathee had said:  ``Corona virus won't spread outside China, we need not worry''  Has this guy ever spoke something sensible? https://t.co/siBAwIR8Pn} %[https://twitter.com/NicoleB_MD/status/1235198085367844869]
    \\
    \textbf{Label:}\enspace\lbl{2.}\,\lbl{NO, probably not of interest}
    \\
    \textbf{Explanation:} The information is not interesting for the general public as it is an opinion and providing statement of someone else.
\end{enumerate}

% \subsection{Harmfulness}
\subsubsection{\textbf{Question 4:}  To what extent does the tweet appear to be harmful to society, person(s), company(s) or product(s)?}

The purpose of this question is to determine if the content of the tweet aims to and can negatively affect society as a whole, specific person(s), company(s), product(s), or spread rumors about them. The content intends to harm or \textit{weaponize the information}\footnote{The use of information as a weapon to spread misinformation and mislead people.}~\citep{broniatowski2018weaponized}.
A rumor involves a form of a statement whose veracity is not quickly verifiable or ever confirmed\footnote{\url{https://en.wikipedia.org/wiki/Rumor}}.

\textbf{Labels:} To categorize the tweets we defined the following labels based on the Likert scale. A higher value means a higher degree of harm. 

\begin{enumerate}
\itemsep-0.2em 
\item \lbl{NO, definitely not harmful}
\item \lbl{NO, probably not harmful}
\item \lbl{not sure}
\item \lbl{YES, probably harmful}
\item \lbl{YES, definitely harmful}
\end{enumerate}

\noindent \textbf{Examples: }

\begin{enumerate}
\item \textit{How convenient but not the least bit surprising from Democrats! As usual they put politics over American citizens. @SpeakerPelosi withheld \#coronavirus bill so DCCC could run ads AGAINST GOP candidates! \#tcot} 
%[https://twitter.com/WILDMANBS/status/1234964593937723395]
\\
\textbf{Label:}\enspace\lbl{5.}\,\lbl{YES, definitely harmful}
\\
\textbf{Explanation:} This tweet is weaponized to target Nancy Pelosi and the Democrats in general.

\item \textit{As we saw over the wkend, disinfo is being spread online about a supposed national lockdown and grounding flights. Be skeptical of rumors. Make sure you’re getting info from legitimate sources. The @WhiteHouse is holding daily briefings and @cdcgov is providing the latest.} %[https://twitter.com/NicoleB_MD/status/12351980853678448}69]
\\
\textbf{Label:}\enspace\lbl{1.}\,\lbl{NO, definitely not harmful}
\\
\textbf{Explanation:} This tweet is informative and gives advice. It does not attack anyone and is not harmful. %and it does not attack anyone. %Hence, it is informative and not harmful.

\end{enumerate}

% \subsubsection{Need of Verification}
\subsubsection{\textbf{Question 5:} Do you think that a professional fact-checker should verify the claim in the tweet?}

It is important to verify a factual claim by a professional fact-checker, as the claim may cause harm to society, specific person(s), company(s), product(s), or some government entities. However, not all factual claims are important or worthwhile to be fact-checked by a professional fact-checker, because it is a time-consuming procedure. Therefore, the purpose is to categorize the tweet using the labels defined below. While doing so, the annotator can rely on the answers to the previous questions. For this question, we defined the following labels to categorize the tweets. 

%This question should be answered based on the answers of the previous questions.

\noindent \textbf{Labels:}
\begin{enumerate}
\itemsep-0.2em 
\item \lbl{NO, no need to check}: the tweet does not need to be fact-checked, e.g., because it is not interesting, a joke, or does not contain any claim.
\item \lbl{NO, too trivial to check}: the tweet is worth fact-checking, however, this does not require a professional fact-checker, i.e., a non-expert might be able to fact-check the claim. For example, one can verify the information using reliable sources such as the official website of the WHO, etc. An example of a claim is as follows: \textit{``The GDP of the USA grew by 50\% last year.''}
\item \lbl{YES, not urgent}: the tweet should be fact-checked by a professional fact-checker, however, it is not urgent or critical;
\item \lbl{YES, very urgent}: the tweet can cause immediate harm to a large number of people, therefore, it should be verified as soon as possible by a professional fact-checker; 
\item \lbl{Not sure}: the content of the tweet does not have enough information to make a judgment. 
%It is recommended to categorize the tweet using this label when the content of the tweet is not understandable at all. For example, it uses a language (i.e., non-English) or references that it is difficult to understand;
\end{enumerate}

\noindent\textbf{Examples:} 
\begin{enumerate}
%     \item \textit{``Wash your hands like you’ve been chopping %jalapeños 
% jalape$\tilde{n}$os and need to change a contact lens'' says BC Public Health Officer Dr. Bonnie Henry re. ways to protect against \#coronavirus \#Covid\_19} 
\item \textit{Things the GOP has done during the Covid-19 outbreak:   - Illegally traded stocks  - Called it a hoax - Blamed it on China  - Tried to bailout big business without conditions  What they haven’t done:   - Help workers  - Help small businesses - Produced enough tests or ventilators}
%[https://twitter.com/Vez_says/status/1235053552315150337]
\\
\textbf{Label:}\enspace\lbl{2.}\,\lbl{YES, very urgent}
\\
\textbf{Explanation:} Clearly, the content of the tweet blames authority, hence, it is important to verify this claim immediately by a professional fact-checker. In addition, the attention of government entities might be required in order to take necessary actions.
\item \textit{ALERT \img{figures/emoticon_example2.png} The corona virus can be spread through internationally printed albums. If you have any albums at home, put on some gloves, put all the albums in a box and put it outside the front door tonight. I'm collecting all the boxes tonight for safety. Think of your health.}
\\
\textbf{Label:}\enspace\lbl{5.}\,\lbl{NO, no need to check}
\\
\textbf{Explanation:} This is a joke and does not need to be checked by a professional fact checker. 
\end{enumerate}


% \subsection{Harmful to Society}
\uline{\textbf{Question 6:} Is the tweet harmful for society and why?}

The purpose of this question is to categorize if the content of the tweet is intended to harm or is weaponized to mislead the society. To identify that we defined the following labels for the categorization. 

\noindent\textbf{Labels:}
\begin{enumerate}[label=\Alph*.]
\itemsep-0.2em 
\item \lbl{NO, not harmful:} the content of the tweet would not harm the society (e.g., \textit{``I like corona beer''}).
\item \lbl{NO, joke or sarcasm:} the tweet contains a joke (e.g., \textit{``If Corona enters Spain, it’ll enter from the side of Barcelona defense''}) or sarcasm (e.g., \textit{```The corona virus is a real thing.' -- Wow, I had no idea!''}).
\item \lbl{not sure:} if the content of the tweet is not understandable enough to judge.
\item \lbl{YES, panic:} the tweet spreads panic. The content of the tweet can cause sudden fear and anxiety for a large part of the society (e.g., \textit{``there are 50,000 cases ov COVID-19 in Qatar''}).
\item \lbl{YES, xenophobic, racist, prejudices, or hate-speech:} the tweet reports xenophobia, racism or prejudiced expression(s). 
According to the dictionary\footnote{\url{https://www.dictionary.com/}} \textit{Xenophobic} refers to fear or hatred of foreigners, people from different cultures, or strangers. \textit{Racism} is the belief that groups of humans possess different behavioral traits corresponding to physical appearance and can be divided based on the superiority of one race over another.\footnote{\url{https://en.wikipedia.org/wiki/Racism}} It may also refer to prejudice, discrimination, or antagonism directed against other people because they are of a different race or ethnicity. \textit{Prejudice} is an unjustified or incorrect attitude (i.e., typically negative) towards an individual based solely on the individual's membership of a social group.\footnote{\url{https://www.simplypsychology.org/prejudice.html}}
An example of a xenophobic statement is \textit{``do not buy cucumbers from Iran''}.
\item \lbl{YES, bad cure:} the tweet reports a questionable cure, medicine, vaccine or prevention procedures (e.g., \textit{``\dots drinking bleach can help cure coronavirus''}). 

\item \lbl{YES, rumor, or conspiracy:} the tweet reports or spreads a rumor. It is defined as a ``specific (or topical) proposition for belief passed along from person to person usually by word of mouth without secure standards of evidence being present''~\citep{allport1947psychology}.  
%A rumor involves a form of a statement whose veracity is not quickly or ever confirmed. 
For example, \textit{``BREAKING: Trump could still own stock in a company that, according to the CDC, will play a major role in providing coronavirus test kits to the federal government, which means that Trump could profit from coronavirus testing. \#COVID-19 \#coronavirus https://t.co/Kwl3ylMZRk''}
\item \lbl{YES, other:} if the content of the tweet does not belong to any of the above categories, then this category can be chosen to label the tweet.

%to this is to cover other cases that need attention.
\end{enumerate}

% \inote{FA: to be consistent with previous questions, do we need examples with label and explanation?}

% \subsection{Requires attention}
\subsubsection{\textbf{Question 7:} Do you think that this tweet should get the attention of any government entity?}

Most often people tweet by blaming authorities, providing advice, and/or call for action. Sometimes that information might be useful for some government entities to make a plan, respond or react on it. The purpose of this question is to categorize such information. It is important to note that not all information requires attention from a government entity. Therefore, even if the tweet's content belongs to any of the positive categories, it is important to understand whether that requires government attention. For the annotation, it is mandatory to first decide on whether attention is necessary from %some 
government entities (i.e., \lbl{YES/NO}). If the answer is \lbl{YES}, it is obligatory to select a category from the \lbl{YES} sub-categories mentioned below.
%Choosing a ``YES:...” answer means that you believe that some government entity should consider the information in the tweet, and possibly respond/react/act on it, use it in planning, etc. 

% Note: Not all blaming of the authorities, calls for actions, discussions of actions taken or of possible cures, and not all questions asked deserve the attention of a government entity. Thus, you should first decide on YES/NO, and in case you think it is a YES, you should select a reason (a category) choosing from the list of YES sub-categories.

\noindent\textbf{Labels:}
\begin{enumerate}[label=\Alph*.]
\itemsep-0.2em 
\item \lbl{NO, not interesting:} if the content of the tweet is not important or interesting for any government entity to pay attention to. 
\item \lbl{not sure:} if the content of the tweet is not understandable enough to judge. 
\item \lbl{YES, categorized as in question 6:} if some government entities need to pay attention to this tweet as it is harmful for society, i.e., it is labeled as any of the \textit{YES} sub-categories in question 6. 
\item \lbl{YES, other:} if the tweet cannot be labeled as any of the above categories, then this label should be selected. 
\item \lbl{YES, blame authorities:} the tweet contains information that blames some government entities or top politician(s), e.g., \textit{``Dear @VP Pence: Is the below true? Do you have a plan? Also, when are local jurisdictions going to get the \#Coronavirus test kits you promised?''}.

\item \lbl{YES, contains advice:} the tweet contains advice about social, political, national, or international issues that requires attention from some government entities (e.g., \textit{The elderly \& people with pre-existing health conditions are more susceptible to \#COVID19. To stay safe, they should: \checkmark Keep distance from people who are sick \checkmark Frequently wash hands with soap \& water \checkmark  Protect their mental health}).
%https://twitter.com/UN/status/1244113301577109505
%about how to fight the virus (e.g., ``wash your hands'')

\item \lbl{YES, calls for action:} the tweet contains information that states that some government entities should take action for a particular issue (e.g., \textit{I think the Government should close all the Barber Shops and Salons , let people buy shaving machines and other beauty gardgets keep in their houses. Salons and Barbershops might prove to be another Virus spreading channels @citizentvkenya @SenMutula @CSMutahi\_Kagwe}).
%https://twitter.com/chakil/status/1244929271749115904
%calls for action (e.g., ``the government should close the barber shops'')

\item \lbl{YES, discusses action taken:} if the tweet discusses actions taken by governments, companies, individuals for any particular issue, for example, closure of bars, conferences, churches due to the corona virus (e.g., \textit{Due to the current circumstances with the Corona virus, The 4th Mediterranean Heat Treatment and Surface Engineering Conference in Istanbul postponed to 26-28 Mayıs 2021.}). 

%%etc. to fight the virus (e.g., closure of bars, conferences, churches, etc.)
\item \lbl{YES, discusses cure:} if attention is needed from some government entities as the tweet discusses a possible cure, vaccine, or treatment for a disease (e.g., \textit{Pls share this valuable information. Garlic boiled water can be cure corona virus}). 

\item \lbl{YES, asks question:} if the content of the tweet contains a question over a particular issue and it requires attention from government entities (e.g., \textit{Special thanks to all doctors and nurses, new found respect for you’ll. Is the virus going to totally disappear in the summer? I live in USA and praying that when the temperature warms up the virus will go away...is my thinking accurate?})
%(e.g., ``Is the virus going to disappear in the summer?'')
%https://twitter.com/Charmai79723273/status/1246505842926587907


\end{enumerate}


==> sections/discussion.tex <==
\section{Discussion}
\label{sec:discussion}
\inote{FA: my observation is that contents in this section are all about data, may be we can move them under data section}

\subsection{Annotation}

When annotating data by multiple people, there is always a risk of discrepancies, which was true also in our case, despite our ongoing efforts to update the instructions and to clarify all confusing/borderline cases we came across. That is why after annotating, we conducted an analysis of the tweet labels based on the common building blocks and categories they might fall in. We noticed several discrepancies in the labels of tweets within the same categories, which we discuss below, with focus on question 5.

One of the most common claim categories for the annotated tweets can be roughly described as \emph{There are X COVID-19 cases at place Y}. These types of claims can be easily verified by visiting an official government website, and thus the most appropriate label for question 5 for them would be \emph{No, too trivial to check}. However, some of the claims from this category were labeled as \emph{Yes, not urgent}, and such labels were corrected during a label consolidation meeting.

Another category that caused contradicting labels concerned the death rate from COVID-19. We must make a clear differentiation in how the claims are stated. For instance, if the tweet says \emph{X percent of people who have fallen ill to COVID-19 have died}, then this claim can be easily checked using officially published COVID-19 data. On the other hand, if the sentence states \emph{The death rate from COVID-19 is X percent}, the claim becomes substantially different: the true death rate of an ongoing disease cannot be easily estimated from a sample of the current death rate statistic. Thus, we labeled such tweets as \emph{Yes, not urgent}.

The next category that initially contained contradictory labels can be described as \emph{The government at place X announced the following measures to tackle the COVID-19 epidemic: ...} Such claims were decided to be categorized as \emph{No, too trivial to check}, since one could easily access the official government site at place $X$ and search for the announcement of the respective measures.

Another category that sparked disagreement within the annotators can be summarized as \emph{Person X has tested positive for COVID-19}. The answer to question 5 for these types of tweets depended on the status of the person in mind. If he or she was a well-known public figure or a high-level politician, then the information was considered of interest to the society, i.e., \emph{Yes} on Q4. If the person in mind was not a public figure and his or her name was mentioned, i.e., due to the fact that he or she is the first person to have tested positive in a certain geographical area, we considered such claims as too trivial to check.

The last category that we will discuss involves tweets with claims revolving around the demonstrative pronoun \emph{this}. We reached an agreement to consider tweets that include \emph{this} as not containing a claim if the claim did not include a URL to an external source or if it was not apparently obvious based on the text who or what the pronoun \emph{this} referred to. If such a tweet was labeled as containing a claim, then it was annotated according to the established instructions.

\inote{FA: the following might raise question, for example, about correcting labels, what is final distribution then?}
In an attempt to automatically detect semantically similar tweets, we converted all examples from the data set to sentence embeddings by mean-pooling the embeddings for each token from BERT. Then, we computed the cosine similarities for each pair of tweets and sorted them in descending order. By doing so, we were able to detect three pairs of semantically similar tweets, one of which had contradicting labels for the other two tweets, and we corrected its label accordingly for the sake of consistency.
\subsection{Correlation Between Questions}
\label{sec:correlation}
%%%%%%%%% English dataset
\begin{figure*}
\centering
    \begin{subfigure}[b]{0.5\textwidth}
        \includegraphics[width=\textwidth]{figures/conf_mat_combined_data_q2_3.png}
        \caption{Heatmap for Q2 and Q3.}
        \label{fig:contingency_table_q2_q3}
    \end{subfigure}%
    \begin{subfigure}[b]{0.5\textwidth}    
        \includegraphics[width=\textwidth]{figures/conf_mat_combined_data_q2_q4.png}
        \caption{Heatmap for Q2 and Q4.}
        \label{fig:contingency_table_q2_q4}    
    \end{subfigure} 
    \hfill
    \begin{subfigure}[b]{0.5\textwidth}    
        \includegraphics[width=\textwidth]{figures/conf_mat_combined_data_q2_q5.png}
        \caption{Heatmap for Q2 and Q5.}
        \label{fig:contingency_table_q2_q5}    
    \end{subfigure}%
    \begin{subfigure}[b]{0.5\textwidth}    
        \includegraphics[width=\textwidth]{figures/conf_mat_combined_data_q3_q4.png}
        \caption{Heatmap for Q3 and Q4.}
        \label{fig:contingency_table_q3_q4}    
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.5\textwidth}    
        \includegraphics[width=\textwidth]{figures/conf_mat_combined_data_q3_q5.png}
        \caption{Heatmap for Q3 and Q5.}
        \label{fig:contingency_table_q3_q5}    
    \end{subfigure}%
    \begin{subfigure}[b]{0.5\textwidth}    
        \includegraphics[width=\textwidth]{figures/conf_mat_combined_data_q4_q5.png}
        \caption{Heatmap for Q4 and Q5.}
        \label{fig:contingency_table_q4_q5}    
    \end{subfigure}     
    \hfill
    \begin{subfigure}[b]{0.5\textwidth}    
        \includegraphics[width=\textwidth]{figures/conf_mat_combined_data_q6_q7.png}
        \caption{Heatmap for Q6 and Q7. YES, X/R/P/HS -- YES, xenophobic, racist, prejudices or hate speech}
        \label{fig:contingency_table_q6_q7}    
    \end{subfigure}%
    \begin{subfigure}[b]{0.5\textwidth}    
            
        \includegraphics[width=\textwidth]{figures/correlation_q2_q4.png}
        \caption{Correlation between Q2 to Q4.}
        \label{fig:english_correlation_q2_q4}

    \end{subfigure}    
    \caption{Contingency and correlation heatmaps of \textbf{English tweets} for different question pairs}
    \label{fig:contingency_all}
\end{figure*}

\begin{figure*} 
\centering
    \begin{subfigure}[b]{0.5\textwidth}
        \includegraphics[width=\textwidth]{figures/arabic_conf_mat_combined_data_q2_q3.png}
        \caption{Heatmap for Q2 and Q3.}
        \label{fig:arabic_contingency_table_q2_q3}
    \end{subfigure}%
    \begin{subfigure}[b]{0.5\textwidth}    
        \includegraphics[width=\textwidth]{figures/arabic_conf_mat_combined_data_q2_q4.png}
        \caption{Heatmap for Q2 and Q4.}
        \label{fig:arabic_contingency_table_q2_q4}    
    \end{subfigure} 
    \hfill
    \begin{subfigure}[b]{0.5\textwidth}    
        \includegraphics[width=\textwidth]{figures/arabic_conf_mat_combined_data_q2_q5.png}
        \caption{Heatmap for Q2 and Q5.}
        \label{fig:arabic_contingency_table_q2_q5}    
    \end{subfigure}%
    \begin{subfigure}[b]{0.5\textwidth}    
        \includegraphics[width=\textwidth]{figures/arabic_conf_mat_combined_data_q3_q4.png}
        \caption{Heatmap for Q3 and Q4.}
        \label{fig:arabic_contingency_table_q3_q4}    
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.5\textwidth}    
        \includegraphics[width=\textwidth]{figures/arabic_conf_mat_combined_data_q3_q5.png}
        \caption{Heatmap for Q3 and Q5.}
        \label{fig:arabic_contingency_table_q3_q5}    
    \end{subfigure}%
    \begin{subfigure}[b]{0.5\textwidth}    
        \includegraphics[width=\textwidth]{figures/arabic_conf_mat_combined_data_q4_q5.png}
        \caption{Heatmap for Q4 and Q5.}
        \label{fig:arabic_contingency_table_q4_q5}    
    \end{subfigure}     
    \hfill
    \begin{subfigure}[b]{0.5\textwidth}    
        \includegraphics[width=\textwidth]{figures/arabic_conf_mat_combined_data_q6_q7.png}
        \caption{Heatmap for Q6 and Q7. YES, X/R/P/HS -- YES, xenophobic, racist, prejudices or hate speech}
        \label{fig:arabic_contingency_table_q6_q7} 
        
    \end{subfigure}%
    \begin{subfigure}[b]{0.5\textwidth}    
        \includegraphics[width=\textwidth]{figures/arabic_correlation_q2_q4.png}
        \caption{Correlation between Q2 to Q4.}
        \label{fig:arabic_correlation_q2_q4}
    \end{subfigure}    
    \caption{Contingency and correlation heatmaps of \textbf{Arabic tweets} for different question pairs }
    \label{fig:arabic_contingency_all}
\end{figure*}

\subsubsection{English Tweets Dataset}
%\textcolor{blue}{nd: may be say more?}
In Figure \ref{fig:contingency_all}, we report the contingency and correlation tables in a form of a heatmap for different question pairs obtained from the English tweet dataset. For questions Q2-3, it appears that there is a high association\footnote{Note that, a Chi-Square test could have been a viable solution to prove such an association, however, our data size is still small (in many cases cell values are less than 5) to do such a test.} between ``\dots no false info'' and the general public interest as shown in Figure  \ref{fig:contingency_table_q2_q3}. For questions Q2 and Q4 %as shown in 
(Figure \ref{fig:contingency_table_q2_q4}), a high association can be observed between ``\dots~no false info'' and ``\dots~not harmful'' (65\%) compared to ``harmful'' (34\%) for either an individual, products or government entities. By analyzing questions Q2 and Q5 (Figure \ref{fig:contingency_table_q2_q5}), we conclude that ``\dots no false info'' is associated with either ``no need to check'' or ``too trivial to check'', highlighting the fact that a professional fact-checker does not need to spend time on them. From questions Q3 and Q4 (Figure \ref{fig:contingency_table_q3_q4}), it appears that when the content of the tweets is ``not harmful'' the general public interest is higher (61\%) than when it is ``harmful'' (39\%).
From question Q3 and Q5 (Figure \ref{fig:contingency_table_q3_q5}), we see an interesting phenomenon, namely tweets with a high general public interest have a greater association with a professional fact-checker having to verify them (61\%) compared to either ``too trivial to check'' or ``no need to check'' (39\%). The questions Q4 and Q5 (Figure \ref{fig:contingency_table_q4_q5}) show that ``harmful'' tweets require more attention (53\%) from a professional fact-checkers than ``not harmful'' tweets (45\%). Our findings for Q6 and Q7 (Figure \ref{fig:contingency_table_q6_q7}) suggest that the majority of the tweets are not harmful for society, which also requires less attention from government entities. The second most common tweet label for Q7 blames authorities, though they are mostly not harmful for society.    

In Figure \ref{fig:english_correlation_q2_q4}, we report the correlation between questions Q2-4 for the English tweets in order to understand their association. We computed the correlation using the Likert scale values (i.e., 1-5) that we defined for these questions. We observed that overall Q2 and Q3 are negatively correlated, which infers that if the claim contains no false information, it is of high interest to the general public. This can be also observed in Figure \ref{fig:contingency_table_q2_q3}. Questions Q2 and Q4 show a positive correlation, which might be due to their high association with ``\dots no false info'' and ``\dots not harmful''.



% \begin{figure}[]
% \centering
% \includegraphics[width=1.0\linewidth]{figures/conf_mat_combined_data_q6_q7.png}
% \caption{Contingency table for Q6 and Q7.}
% \label{fig:contingency_q6_q7}
% \end{figure}

% \begin{figure}[]
% \centering
% \includegraphics[width=0.8\linewidth]{figures/correlation_q2_q4.png}
% \caption{Spearman rank correlation between questions Q2 to Q4. Computed using Likert values associated with the labels of these questions.}
% \label{fig:contingency_q6_q7}
% \end{figure}



%%%%%%%%%% Arabic dataset
% \subsubsection*{Arabic Tweets Dataset}
\subsubsection{Arabic Tweets Dataset}
% \inote{to discuss figures (contingency and correlation)}
In Figure \ref{fig:arabic_contingency_all}, we report heatmaps to illustrate the association across questions using the Arabic tweets. From Q2 and Q3 (Figure \ref{fig:arabic_contingency_table_q2_q3}), we can observe that the association between ``\dots contains no false info'' and general public interest is higher (67\%) than ``\dots contains false info'' (29\%). From questions Q2 and Q4 (Figure \ref{fig:arabic_contingency_table_q2_q4}), we conclude that ``\dots contains no false info'' is associated with ``\dots not harmful'' and ``\dots contains false info'' is associated with ``\dots harmful'', which can also be established from its high correlation of 0.74 in Figure \ref{fig:arabic_correlation_q2_q4}. From the relation between Q2 and Q5 (Figure \ref{fig:arabic_contingency_table_q2_q5}), it can be seen that in the majority of the cases ``\dots contains no false info'' is associated with either ``no need to check'' or ``too trivial to check'', which means that a professional fact-checker does not need to verify them. The analysis between questions Q3 and Q4 suggests that general public interest is higher when the content of the tweets is not harmful (68\%) than harmful (30\%) (Figure \ref{fig:arabic_contingency_table_q3_q4}). From questions Q3 and Q5, we can observe that the general public interest is higher when the claim(s) in the tweets are either ``no need to check'' or ``too trivial to check'' (Figure \ref{fig:arabic_contingency_table_q3_q5}). 
%From 
The analysis between question Q4 and Q5 shows that ``not harmful'' tweets are either ``no need to check'' or ``too trivial to check'' by a professional fact-checker (Figure \ref{fig:arabic_contingency_table_q4_q5}). From the questions Q6 and Q7, we notice that in the majority of the cases the tweets are not harmful for society and hence they are not interesting for government entities (Figure \ref{fig:arabic_contingency_table_q6_q7}).  



% \begin{figure*} 
% \centering
%     \begin{subfigure}[b]{0.60\textwidth}
%         \includegraphics[width=\textwidth]{figures/Rplot_Answers4EngQs.pdf}
%         \caption{English dataset}
%         \label{fig:english_data_with_users}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[b]{0.60\textwidth}    
%         \includegraphics[width=\textwidth]{figures/Rplot_Answers4AraQs.pdf}
%         \caption{Arabic dataset}
%         \label{fig:arabic_data_with_users}    
%     \end{subfigure} 
% \caption{Distribution of datasets for all the questions associated with user accounts. NA refers to tweets that have not been labeled for those questions, they are identical to the tweets categorized with the label NO in Q1.}
% \label{fig:user_account_label_dist}
% \end{figure*}









